Disentangled Recurrent Wasserstein Autoencoder

Learning disentangled representations leads to interpretable models and facilitates data generation with style transfer, which has been extensively studied on static data such as images in an unsupervised learning framework. However, only a few works have explored unsupervised disentangled sequential representation learning due to challenges of generating sequential data. In this paper, we propose recurrent Wasserstein Autoencoder (R-WAE), a new framework for generative modeling of sequential data. R-WAE disentangles the representation of an input sequence into static and dynamic factors (i.e., time-invariant and time-varying parts). Our theoretical analysis shows that, R-WAE minimizes an upper bound of a penalized form of the Wasserstein distance between model distribution and sequential data distribution, and simultaneously maximizes the mutual information between input data and different disentangled latent factors, respectively. This is superior to (recurrent) VAE which does not explicitly enforce mutual information maximization between input data and disentangled latent representations. When the number of actions in sequential data is available as weak supervision information, R-WAE is extended to learn a categorical latent representation of actions to improve its disentanglement. Experiments on a variety of datasets show that our models outperform other baselines with the same settings in terms of disentanglement and unconditional video generation both quantitatively and qualitatively.

==> tex/experiments.tex <==
\begin{figure*}
\begin{center}
\begin{subfigure}{0.33333\textwidth}
\centering
\begingroup
\begin{tabular}{cccc}
\includegraphics[height=.197\textwidth]{figures/6P0fram0.png} & \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6P0fram9.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6P0fram49.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6P0fram99.png} \\
\includegraphics[height=.197\textwidth]{figures/6SF0fram0.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6SF0fram9.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6SF0fram49.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6SF0fram99.png} \\
\includegraphics[height=.197\textwidth]{figures/6SZ0fram0.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6SZ0fram9.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6SZ0fram49.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6SZ0fram99.png} \\
\includegraphics[height=.197\textwidth]{figures/6P1fram0.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6P1fram9.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6P1fram49.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/6P1fram99.png} \\
\end{tabular}
\endgroup
\vspace{-0.2cm}
\caption{t=1;~~ t=10;~~ t=50;~~ t=100} 
\end{subfigure}
\hspace{-.3cm}
\begin{subfigure}{0.33333\textwidth}
\centering
\begingroup
\begin{tabular}{cccc}
\includegraphics[height=.197\textwidth]{figures/5P0fram0.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5P0fram2.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5P0fram4.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5P0fram6.png}\\
\includegraphics[height=.197\textwidth]{figures/5SF0fram0.png}&\hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5SF0fram2.png}&\hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5SF0fram4.png}&\hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5SF0fram6.png}\\ 
\includegraphics[height=.197\textwidth]{figures/5SZ0fram0.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5SZ0fram2.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5SZ0fram4.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5SZ0fram6.png}\\ 
\includegraphics[height=.197\textwidth]{figures/5P1fram0.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5P1fram2.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5P1fram4.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/5P1fram6.png}\\ 
\end{tabular}
\endgroup
\vspace{-0.2cm}
\caption{t=1;~~ t=3;~~ t=5;~~ t=7}
\end{subfigure}
\hspace{-.3cm}
\begin{subfigure}{0.33333\textwidth}
\centering
\begingroup
\begin{tabular}{cccc}
 \includegraphics[height=.197\textwidth]{figures/15P0fram0.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15P0fram2.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15P0fram4.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15P0fram6.png}\\
\includegraphics[height=.197\textwidth]{figures/15SZ0fram0.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15SZ0fram2.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15SZ0fram4.png}& \hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15SZ0fram6.png} \\
\includegraphics[height=.197\textwidth]{figures/15SF0fram0.png}&\hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15SF0fram2.png}&\hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15SF0fram4.png}&\hspace{-0.4cm}
\includegraphics[height=.197\textwidth]{figures/15SF0fram6.png} \\
\includegraphics[height=.197\textwidth]{figures/15P1fram0.png}& \hspace{-0.3cm}
\includegraphics[height=.197\textwidth]{figures/15P1fram2.png}& \hspace{-0.3cm}
\includegraphics[height=.197\textwidth]{figures/15P1fram4.png}& \hspace{-0.3cm}
\includegraphics[height=.197\textwidth]{figures/15P1fram6.png} \\
\end{tabular}
\endgroup
\vspace{-0.2cm}
\caption{t=1; t=3; t=5; t=7} 
\end{subfigure}
\vspace{-0.2cm}
\caption{Illustration of disentangling the motions and contents of two randomly chosen sequences on the test data of SM-MNIST (left, $T=100$), Sprites (middle, $T=8$) and MUG dataset (right, $T=8$). The first row and fourth row are original video sequences. The second row and third row are reconstructed videos by swapping the respective content and motion from the first row and fourth row. \label{fig:distoy}}
\end{center}
\end{figure*}



\section{Experiments}
We conduct extensive experiments on four datasets to quantitatively and qualitatively validate our methods.  %We compare our methods with 
The baseline methods for comparisons are DS-VAE~\cite{li2018disentangled} and MoCoGAN~\cite{tulyakov2018mocogan}. We train our models on Stochastic moving MNIST (SM-MNIST), Sprites and TIMIT datasets under a completely unsupervised setting. The number of actions is used as the prior information for all methods on MUG facial dataset. The detailed descriptions of datasets, architectures and hyperparameters are provided in Appendix C, D, E, respectively.  
% \begin{minipage*}{\textwidth}
% \begin{minipage}[h]{0.28\textwidth}  %0.31

% \begin{figure}[htb]
% \centering
%  \includegraphics[height=0.26\textwidth]{figures/latent_mmd_long_final.pdf}
%   \vspace{-0.5cm}
%     \captionof{figure}{2D manifold of the content latent code $\{\vz^c\}$ encoded from R-WAE(MMD) on SM-MNIST by t-SNE~\cite{maaten2008visualizing}. \label{manifold}}
% %   \end{minipage}
% %   \hfill \hspace{-0.1cm}
% \end{figure}
%   \begin{minipage}[bth]{0.68\textwidth}  %0.68
% \begin{table}
% \centering
% \begin{tabular}{|p{1.55cm}|p{.8cm}|p{1.35cm}|p{.6cm}|p{.65cm}|p{.55cm}|}
%  \hline
% \multirow{2}{*}{\!\!\!\backslashbox{\! {\small Methods}}{\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! {\small \!\! Datasets}}}& \multicolumn{4}{|c|}{ Sprites}& \multicolumn{1}{|c|}{{\small MNIST}} \\
%  \cline{2-6}
%  & actions & {\small skin color} & pants & tops & digits\\
%  \hline
% {\small DS-VAE(S)} &  8.11\%  & 3.98\% & 1.82\% &  0.34\% & 3.31\%\\ \hline
% R-WAE(S) & {\bf 5.83\%} & {\bf 2.45\%}  & 1.73\%   & 0.32\% & {\bf 1.78\%} \\
%  \hline
% {\small DS-VAE(C)} & 10.37\%  & 4.86\% & 3.62\% &  0.53\% & 4.26\% \\ \hline
% R-WAE(C) & {\bf 7.72\%} & {\bf 3.31\%}  & 3.20\%   & 0.40\% & {\bf 2.84\%} \\
%  \hline 
% \end{tabular}
% \vspace{-0.2cm}
% \captionof{table}{Comparison of averaged classification errors. For Sprites dataset, fix one encoded attribute and randomly sample others. For SM-MNIST dataset, we fix the encoded content variable $\vz^c$ and randomly sample the motion sequence from the learned prior $p_{\psi}(\vz_t^m|\vz_{<t}^m).$ No label of motions on SM-MNIST is available and therefore we cannot verify the motion disentanglement by the accuracy. Lower values indicate better disentanglement.\label{toy:quant}}
% \end{table}
% \end{minipage}
% \end{minipage*}
 
% \subsection{Results on SM-MNIST and Sprites Datasets}
{\bf Qualitative Results on Disentanglement}. MoCoGAN~\cite{tulyakov2018mocogan} is not tailored for SM-MNIST dataset since their training requires finite number of actions in order to disentangle the action. The fact that MoCoGAN doesn't perform well on SM-MNIST can be easily seen from Fig.~\ref{fig:mnistsample}. We find that the performance of MoCoGAN~\cite{tulyakov2018mocogan} is much worse than DS-VAE~\cite{li2018disentangled} and our R-WAE(MMD) on SM-MNIST and Sprite. On MUG dataset, our model can swap the smile and fear action between two persons.   

\begin{minipage}{\textwidth}
\begin{minipage}[h]{0.46 \textwidth}
\begin{center}
\begin{tabular}{|p{1.66cm}|p{1.39cm}|p{1.396cm}|}
\hline
\multirow{2}{*}{\!\!\backslashbox{\! {\small }}{\!\!\!\!\!\!\!\! {\small Metric}}{\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! {\small Methods} }} & \multicolumn{2}{|c|}{~~ERR~} \\ 
 \cline{2-3}
 & \!\! $\vz^c=16$ \!\! $\downarrow$ &\!\!\!\!$\vz^m=16$\!\! $\uparrow$\\ \hline
{\small ~~FHVAE} &  5.06\% & 22.77\%  \\ \hline
{\small ~~DS-VAE} &  4.82\% & 17.84\% \\ \hline
{\small \!\! R-WAE} & {\bf 4.73\%} & {\bf 23.41\%} \\ \hline
\end{tabular}
\captionof{table}{EER on TIMIT speech dataset for the same dimension setting of segment-level $\vz^c$ and sequence-leve $\vz^m$ for FHVAE~\cite{hsu2017unsupervised}, DS-VAE~\cite{li2018disentangled} and R-WAE(MMD), respectively. \label{table:speech}}
\end{center}
\end{minipage}
\begin{minipage}[bth]{0.53 \textwidth}
    \centering
  \begin{tabular}{|p{1.65cm}|p{.8cm}|p{1.32cm}|p{.6cm}|p{.6cm}|p{.4cm}|}
 \hline
  \multirow{2}{*}{\!\!\!\backslashbox{\! {\small Methods}}{\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! {\small \!\! Datasets}}}& \multicolumn{2}{|c|}{ Sprites}& \multicolumn{1}{|c|}{{\small MNIST}} \\
 \cline{2-4}
 & actions & {\small content} & digits \\
 \hline
{\small DS-VAE(S)} &  8.11\%  & 3.98\%  & 3.31\% \\ \hline
R-WAE(S) & {\bf 5.83\%} & {\bf 2.45\%} & {\bf 1.78\%} \\
 \hline
{\small DS-VAE(C)} & 10.37\%  & 4.86\% & 4.26\% \\ \hline
R-WAE(C) & {\bf 7.72\%} & {\bf 3.31\%} & {\bf 2.84\%} \\
 \hline
\end{tabular}  
\captionof{table}{Comparison of averaged classification errors. For Sprites dataset, fix one encoded attribute and randomly sample others. For SM-MNIST dataset, we fix the encoded content variable $\vz^c$ and randomly sample the motion sequence from the learned prior $p_{\psi}(\vz_t^m|\vz_{<t}^m).$ No label of motions on SM-MNIST is available and therefore we cannot verify the motion disentanglement by the accuracy. Lower values indicate better disentanglement.\label{toy:quant}}
\end{minipage}
\end{minipage}

\paragraph{Results on TIMIT Speech Dataset} We quantitatively compare our R-WAE with FHVAE~\cite{hsu2017unsupervised} and DS-VAE \cite{li2018disentangled} under the same setting as \cite{hsu2017unsupervised,li2018disentangled}. The evaluation metric of all methods is based on equal error rate (EER), which is explained in detail in Appendix C. The lower ERR on  $\vz^c$ is better and the higher ERR on $\vz^m$ is expected to be better. From Table~\ref{table:speech}, our model can disentangle the segment-level attribute $\vz^c$ and sequence-leve attribute $\vz^m$ well. We can see that our R-WAE(MMD) has best ERR rate. 


\input{tex/mnist_video.tex}

\paragraph{Qualitative Results on SM-MNIST and Sprites Datasets} We encode videos $A$ and $B$ and reconstruct videos from swapped $\{\vz^c, \vz^m_{1:T}\}$. Results in Fig.~\ref{fig:distoy} are randomly chosen from the test data. Fig.~\ref{fig:distoy}(left) shows that even testing on the long sequence (trained with $T=8$), our R-WAE can disentangle content and motions. It is interesting to observe that digit "7" keeps the same while the shape of digit "8" varies a little bit. In Fig.~\ref{fig:distoy}(right), we do the same swapping on Sprites. We can see that the reconstructed swapped videos have exact same appearances and actions as the corresponding original ones.     

% \begin{figure*}[htb]
% \begin{center}
% \begin{tabular}{cccccccc}
% \rotatebox{0}{{\small ~~~~Original A~~~~~~~}}
% \includegraphics[height=.07\textwidth]{figures/15P0fram0.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15P0fram2.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15P0fram4.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15P0fram6.png}& \hspace{0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7P0fram1.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7P0fram3.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7P0fram5.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7P0fram7.png}\\ \vspace{-0.05cm}
% \rotatebox{0}{{\small $\mathrm{A:}~\vz^R~ \mathrm{and} ~\mathrm{B:}~\vz^c$~}}
% \includegraphics[height=.07\textwidth]{figures/15SZ0fram0.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15SZ0fram2.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15SZ0fram4.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15SZ0fram6.png}& \hspace{0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7SZ0fram1.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7SZ0fram3.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7SZ0fram5.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7SZ0fram7.png}\\ \vspace{-0.05cm}
% \rotatebox{0}{{\small $\mathrm{A:}~\vz^c ~\mathrm{and} ~\mathrm{B:}~\vz^R$~}}
% \includegraphics[height=.07\textwidth]{figures/15SF0fram0.png}&\hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15SF0fram2.png}&\hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15SF0fram4.png}&\hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15SF0fram6.png}&\hspace{0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7SF0fram1.png}&\hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7SF0fram3.png}&\hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7SF0fram5.png}&\hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7SF0fram7.png}\\ \vspace{-0.05cm}
% \rotatebox{0}{{\small ~~~~Original B~~~~~~~}}
% \includegraphics[height=.07\textwidth]{figures/15P1fram0.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15P1fram2.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15P1fram4.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/15P1fram6.png}& \hspace{0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7P1fram1.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7P1fram3.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7P1fram5.png}& \hspace{-0.3cm}
% \includegraphics[height=.07\textwidth]{figures/7P1fram7.png} \\
% \vspace{-0.2cm}
%  {\small ~~~~~~~~~~~~~~~~~~~~~~~~~~~t=1}&{\small t=3}&{\small t=5}&{\small t=7}& {\small t=1}&{\small t=3}&{\small t=5}&{\small t=7} \\
% \end{tabular}
% \vspace{-0.2cm}
% \caption{Illustration of disentangling motions and contents of two sets of sequences ($T=10$) on test data of the MUG. Each video sequence $\vx_{1:T}$ from the original $A$ and $B$ in either left or right is encoded by our model to get $\vz^c$ and $\{\vz_{t}^R\}_{t=1}^T$, where $\vz_{t}^R=(\vz_{t}^m, \va).$ Then we reconstruct videos by swapped $\{\vz^c, \vz_{t}^R\}_{t=1}^T.$\label{fig:dismug}} 
% \end{center}
% \end{figure*}


% \begin{figure}[htb]
% \centering
%  \includegraphics[height=0.26\textwidth]{figures/latent_mmd_long_final.pdf}
%   \vspace{-0.5cm}
%     \captionof{figure}{Visualization of 2D manifold of the content latent code $\{\vz^c\}$ encoded from R-WAE(MMD) on SM-MNIST by t-SNE~\cite{maaten2008visualizing}. \label{manifold}}
% %   \end{minipage}
% %   \hfill \hspace{-0.1cm}
% \end{figure}

\paragraph{Quantitative Results} We quantitatively evaluate the disentanglement of our R-WAE(MMD). In Table ~\ref{toy:quant}, "S" denotes a simple encoder/decoder architecture, where the encoders in both our model and DS-VAE~\cite{li2018disentangled} only use 5 layers of convolutional and deconvolutional networks adopted from DS-VAE~\cite{li2018disentangled}. "C" denotes a complex encoder/decoder architecture where we use Ladder network~\cite{sonderby2016ladder, zhao2017learning} and ResBlock~\cite{he2016deep}, provided in Appendix E. On SM-MNIST, we get the labeled latent codes $\{\vz^c\}$ of test videos $\{\vx_{1:T}\}$ with $T=10$ and randomly sample motion variables $\{\vz^m_{1:T}\}$ to get labeled new samples. We pretrain a classifier and predict the accuracy on these labeled new samples. The accuracy on SM-MNIST dataset is evaluated on 10000 test samples. On Sprites, the labels of each attribute(skin colors, pants, hair styles, tops and pants) are available. We get the latent codes by fixing one attribute and randomly sample other attributes. We train a classifier for each attribute and evaluate the disentanglement of each attribute. The accuracy is based on $296\times 9$ test data. Both DS-VAE and R-WAE(MMD) have extremely high accuracy (99.94\%) when fixing hair style attribute, which is not provided in Table~\ref{toy:quant} due to space limit. There are two interesting observations in Table ~\ref{toy:quant}. First, the simple architecture typically has a better disentanglement than the complex architecture. The reason is that the simple architecture has sufficient ability to extract features and generate clear samples to be recognized by the pretrained classifiers. But the simple architecture cannot generate high-quality samples when applied to real data. Second, our proposed R-WAE(MMD) achieve better disentanglement than DS-VAE~\cite{li2018disentangled} on both corresponding architectures. The attributes within content latent variables are independent, our model can further disentangle the factors.    

As the number of motions in SM-MNIST is infinite and random, we cannot evaluate the disentanglement of motions by training a classifier. We fix the encoded motions $\{\vz^m_{1:T}\}$ and randomly sample content variables $\{\vz^c\}.$ We also randomly sample a motion sequence $\{\vz^m_{1:T}\}$ and randomly sample contents $\{\vz^c\}$. We manually check the motions of these samples and almost all have the same corresponding motion even though the sequence is long ($T=100$).  

\paragraph{Unconditional Video Generation} Fig.~\ref{fig:mnistsample} provides generated samples on SM-MNIST dataset by randomly sampling content $\{\vz^c\}$ from the prior $p(\vz^c)$ and motions $\{\vz^m_{1:T}\}$ from the learned prior $p_\psi(\vz_t^m|\vz_{<t}^m).$ The length of our generated videos is $T=100$ and we only show randomly chosen videos of $T=20$ to save file size. Our R-WAE(MMD) achieves the most consistent and visually best sequence even when $T=100$. Samples from MoCoGAN~\cite{tulyakov2018mocogan} usually change digit identity along the sequence. The reason is that MoCoGAN~\cite{tulyakov2018mocogan} requires the number of actions be finite. Our generated Sprites videos also have the best results but are not provided to save space.  

\begin{table*}
\begin{center}
\resizebox{1\textwidth}{!}{
  \begin{tabular}{|p{2.2cm}|p{1.5cm}|p{2.2cm}|p{1.9cm}|p{2.22cm}|p{2.2cm}|} \hline
\backslashbox{{\small Metrics}}{\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! {\small Methods}} &{\small MocoGAN} & {\small DS-VAE(NA)}& {\small DS-VAE(W)} &{\small R-WAE(MMD)}&{\small R-WAE(GAN)}\\ \hline
 {\small Accuracy ~$\uparrow$} & 75.50\%  & 66.73\% & 82.84 \% & 88.62\% & {\bf 90.15\%}   \\ \hline
 {\small Intra-entropy$\downarrow$} & 0.26 & 0.28& 0.23 & 0.17 & {\bf 0.15} \\ \hline
{\small Inter-entropy$\uparrow$} & 1.78 & 1.77 & 1.78 & {\bf 1.79} & {\bf 1.79}\\ \hline
{\small ~~~~~ IS~$\uparrow$} & 4.60 & 4.44 & 4.71 & 5.05 & {\bf 5.16}  \\ \hline
{\small ~~~ FID~$\downarrow$} & 16.95& 18.72&14.79& {\bf 12.21}& {\bf 10.86} \\
\hline
 \end{tabular}}
\vspace{-0.3cm}
 \caption{Quantitative results on generated samples from the MUG facial dataset. "DS-VAE(NA)" means that number of actions is not incorporated~\cite{li2018disentangled}. In "DS-VAE(NA)", samples are generated by fixing the encoded motions and randomly sampling content variable from the prior. Samples on DS-VAE(W), R-WAE(MMD) and R-WAE(GAN) are generated by incorporating the prior information(number of actions) into the model. \label{quant:mug}} 
 \end{center}
 \end{table*}
 
% \subsection{Results on MUG Facial Dataset}
\paragraph{Results on MUG Facial Dataset} Like MoCoGAN~\cite{tulyakov2018mocogan}, we leverage the prior information (number of actions is 6) to reinforce disentanglement. We incorporate a latent action variable $\va$ (a one-hot vector with dimension 6) into our model to enhance disentanglement. The regularization for learning $\va$ is described in Section \ref{mainmethod}. The latent motion variable is augmented as $\vz^R_t=(\va, \vz^m_t).$

 \input{tex/mug_video.tex}  
% \paragraph{Qualitative Results} we reconstruct videos by swapped encoded codes $\{\vz^c, \vz_t^R\}$ of video $A$ and $B$ on test data in Fig.~\ref{fig:dismug}. We randomly choose two sets of video sequences to illustrate the disentanglement. In Fig.~\ref{fig:dismug} (left), the identity changes from the fear expression to the happy expression or reverse. In Fig.~\ref{fig:dismug} (right), the identity changes from the happy expression to the anger expression or reverse. 

\paragraph{Quantitative Results} We quantitatively evaluate the disentanglement and quality of generated samples. We train a 3D classifier on MUG facial dataset with accuracy 95.11\% and inception score (IS) 5.20 on test data~\cite{salimans2016improved}. We calculate IS, inter-entropy $H(y|\bd{v})$, where $y$ is the predicted label and $\bd{v}$ is the generated video, and intra-entropy $H(y)$. For a comprehensive quantitative evaluation, Frame-level FID score, introduced by~\cite{heusel2017gans}, is also provided. From Table 2, our R-WAE(MMD) and R-WAE(GAN) have higher accuracy, which means the categorical variable best captures the actions, which indicates our models achieves best disentanglement. In table 2, the IS score of R-WAE(GAN) is very close to IS of the exact test data, which means our models have best sample quality. Our proposed R-WAE(GAN) and R-WAE(MMD) have best frame-level FID scores, compared with DS-VAE and MoCoGAN. The orignal DS-VAE (DS-VAE(NA))~\cite{li2018disentangled} without leveraging the number of actions performs worst. It is expected that incorporating the number of actions as prior information enhances the disentanglement of actions. % \textbf{Erran: the following sentence does not parse; needs to be rewritten} 
 
\paragraph{Unconditional Video Generation} Fig.~\ref{fig:mugframe} and Fig.~\ref{fig:mugsample} on the appendix E show generated samples on MUG facial dataset by randomly sampling content $\{\vz^c\}$ from the prior $p(\vz^c)$ and motions $\vz^R_t=(\va, \vz_t^m)$ from the categorical prior $p(\va)$ and the learned prior $p_{\psi}(\vz_t^m|\vz_{<t}^m).$ We show generated videos of length $T=10$ in the Fig.~\ref{fig:mugsample} on the appendix E. DS-VAE~\cite{li2018disentangled} using the same structure as ours. Fig.~\ref{fig:mugsample} shows that DS-VAE~\cite{li2018disentangled} and MoCoGAN~\cite{tulyakov2018mocogan} have blurry first frames $\{\vx_t\}$ and even more blurry frames as the time $t$ evolves. While our R-WAE(GAN) has much better frame quality and much more consistent video sequences. To have a clear comparison among all three methods, we show the sample at time step $T=10$. In Fig.~\ref{fig:mugframe}, we can see that DS-VAE has very blurry sample at large time steps.  

% \begin{figure}[tbh]
% \centering
% \begingroup
% \setlength{\tabcolsep}{.3pt}
% \begin{tabular}{cc}
%  \multicolumn{2}{c}{{\small R-WAE~(MMD)}} \vspace{-.1cm}\\ \vspace{-.15cm} 
% \includegraphics[height=0.199\textwidth]{figures/latent_wae.pdf}& 
% \includegraphics[height=0.199\textwidth]{figures/latent_wae_long.pdf} \\
% {\small (a) 100 Epochs} & {\small (b) 500 Epochs} \\
% \end{tabular}
% \begin{tabular}{cc}
% \multicolumn{2}{c}{{\small Li\&Mandt, 2018}} \vspace{-.1cm} \\ \vspace{-.15cm} 
% \includegraphics[height=0.199\textwidth]{figures/latent_kl.pdf} &
% \includegraphics[height=0.199\textwidth]{figures/latent_kl_long.pdf}\\
% {\small (c) 100 Epochs} & {\small (d) 500 Epochs} \\
% \end{tabular}
% \endgroup
% \caption{\small Visualization of latent manifolds on SM-MNIST dataset. The static parts of both methods can learn the invariant digit information in the beginning training epochs. It is interesting to observe that Li\&Mandt tends to collapse after long training while ours are stable. \label{fig:latent}}
% \end{figure}



==> tex/mnist_video.tex <==
% \iffalse
% \begin{figure*}[thb]
% \centering

% \begin{subfigure}{.33\textwidth}
% \centering
% \begin{tabular}{ccccc}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/0G1fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/2G0fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/2G1fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/3G0fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/13G0fram}{0}{19} \\ 
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/4G0fram}{0}{19}& \hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/11G0fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/02G1fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/05G0fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/6G0fram}{0}{19}\\ 
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/6G1fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/04G0fram}{0}{19}&\hspace{-0.5cm} 
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/7G0fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/7G1fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/07G0fram}{0}{19} \\
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/8G0fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/08G0fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/8G1fram}{0}{19}&\hspace{-0.5cm}  
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/10G1fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/5G0fram}{0}{19}\\ 
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/15G1fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/14G0fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/14G1fram}{0}{19}&\hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/12G0fram}{0}{19}& \hspace{-0.5cm}
% \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/02G0fram}{0}{19}\\
% \end{tabular}
% \vspace{-0.2cm}
% \caption{R-WAE(MMD)}
% \end{subfigure}

% \iffalse
%   \begin{subfigure}{.33\textwidth}
%   \centering
%   \begin{tabular}{ccccc}
%   \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/01G0fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/1G0fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/1G1fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/2G1fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/18G0fram}{0}{19}\\
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/19G0fram}{0}{19}& \hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/3G1fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/03G0fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/26G1fram}{0}{19}&\hspace{-0.5cm} 
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/5G1fram}{0}{19}\\
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/7G0fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/7G1fram}{0}{19}& \hspace{-0.5cm} 
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/8G1fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/11G1fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/2G0fram}{0}{19}\\
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/12G1fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/13G0fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/13G1fram}{0}{19}& \hspace{-0.5cm} 
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/15G0fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/17G1fram}{0}{19}\\
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/16G0fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/16G1fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/19G1fram}{0}{19}& \hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/12G0fram}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{VAE_MNIST/3G0fram}{0}{19}\\
%  \end{tabular}
%  \caption{DS-VAE~\cite{li2018disentangled}} 
%  \end{subfigure}
% \hspace{-.3cm}

%  \begin{subfigure}{.33\textwidth}
%  \centering
%  \begin{tabular}{ccccc}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{mocogan_smmnist/0_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{mocogan_smmnist/1_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{mocogan_smmnist/2_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{mocogan_smmnist/3_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.185\textwidth]{2}{mocogan_smmnist/4_smmnist_}{0}{19}\\ 
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/5_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/6_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/7_smmnist_}{0}{19}&\hspace{-0.5cm} 
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/8_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/9_smmnist_}{0}{19} \\
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/10_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/11_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/12_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/13_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/14_smmnist_}{0}{19} \\
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/15_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/16_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/17_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/18_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/19_smmnist_}{0}{19} \\
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/20_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/21_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/22_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/23_smmnist_}{0}{19}&\hspace{-0.5cm}
%  \animategraphics[loop,autoplay,height=.18\textwidth]{2}{mocogan_smmnist/24_smmnist_}{0}{19} \\ 
%  \end{tabular}
%  \vspace{-0.2cm}
%  \caption{MoGoGAN \cite{tulyakov2018mocogan}} 
%  \end{subfigure}
% \fi

% \vspace{-0.2cm}
% % \caption{Unconditional video generation on SM-MNIST. (a), sequences (length=20) in R-WAE(MMD) are randomly taken from generated samples with $T=100$ to save pdf size. (b), generated videos by DS-VAE~\cite{li2018disentangled} with $T=20$. (c), generated videos by MoCoGAN~ \cite{tulyakov2018mocogan} with $T=20$. Viewed with Adobe Reader to see video. \label{fig:mnistsample}
% \caption{Unconditional video generation on SM-MNIST. (a), sequences (length=20) in R-WAE(MMD) are randomly taken from generated samples with $T=100$ to save pdf size. \label{fig:mnistsample}
% %\textbf{Erran: (b) and (c) are missing}
% } 
% \end{figure*}
% % \fi


\begin{figure*}[h]
    \centering
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{ccccc}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/0G1fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/2G0fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/2G1fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/3G0fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/13G0fram}{0}{19} \\ 
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/4G0fram}{0}{19}& \hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/11G0fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/02G1fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/05G0fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/6G0fram}{0}{19}\\ 
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/6G1fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/04G0fram}{0}{19}&\hspace{-0.5cm} 
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/7G0fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/7G1fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/07G0fram}{0}{19} \\
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/8G0fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/08G0fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/8G1fram}{0}{19}&\hspace{-0.5cm}  
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/10G1fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/5G0fram}{0}{19}\\ 
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/15G1fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/14G0fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/14G1fram}{0}{19}&\hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/12G0fram}{0}{19}& \hspace{-0.5cm}
    \animategraphics[loop,autoplay,height=.185\textwidth]{2}{figures/02G0fram}{0}{19}\\
    \end{tabular}}
    \caption{Unconditional video generation on SM-MNIST. Sequences (length=20) in R-WAE(MMD) are randomly taken from generated samples with $T=100$ to save pdf size. \label{fig:mnistsample}}
\end{figure*}
